Stream attention-based multi-array end-to-end speech recognition

Automatic Speech Recognition (ASR) using multiple microphone arrays has achieved great success in the far-field robustness. Taking advantage of all the information that each array shares and contributes is crucial in this task. Motivated by the advances of joint Connectionist Temporal Classification (CTC)/attention mechanism in the End-to-End (E2E) ASR, a stream attention-based multi-array framework is proposed in this work. Microphone arrays, acting as information streams, are activated by separate encoders and decoded under the instruction of both CTC and attention networks. In terms of attention, a hierarchical structure is adopted. On top of the regular attention networks, stream attention is introduced to steer the decoder toward the most informative encoders. Experiments have been conducted on AMI and DIRHA multi-array corpora using the encoder-decoder architecture. Compared with the best single-array results, the proposed framework has achieved relative Word Error Rates (WERs) reduction of 3.7% and 9.7% in the two datasets, respectively, which is better than conventional strategies as well.

==> intro_new.tex <==
% 3. description of end-to-end approach and its advantage. Introduction of joint e2e model.prior work in e2e (multi-array and multi-channel)  --ruizhili 
The end-to-end speech recognition is developed to directly transcribe human speech into text. 
It integrates disjoint modules, developed from traditional hybrid methods, into one single Deep Neural Network (DNN) which can be trained from scratch.
The attention-based structure \cite{} solves the ASR problem as a sequence mapping by using an encoder-decoder architecture. 
Coupled with a Connectionist Temporal Classification (CTC) network  \cite{}, the joint model \cite{} outperforms the attention-based ASR by addressing misalignment issues. 
While most of the end-to-end ASR studies engage in single-channel(microphone) task \cite{} or multi-channel task from one microphone array \cite{}, research on multi-array scenario is still unexplored within end-to-end framework. 


% 4. porposed specially, how fusion is done(frame-level fusion(multi-head), context vector level fusion(HAN)) --ruizhi
In this work, we propose a multi-stream architecture followed by a hierarchical attention mechanism for the fusion of stream-level information. 


to solve the multiple array ASR problem using the advanced E2E systems - the joint CTC/attention framework. 
The output of each microphone array is modeled by a separate encoder. 
On top of the per-encoder attention mechanism, hierarchical attention network is employed to focus on the array stream that generates more informative higher-level representations. 
At the same time, each encoder is associated with a CTC network to guide the frame-wise alignment process, in order to potentially achieve the best results. 





encoder-fusion (frame-level)
encoder fusion end-to-end frame0-level contect level end-to-end


In this work, we propose a multi-stream architecture to solve the multiple array ASR problem using the advanced E2E systems - the joint CTC/attention framework. 
The output of each microphone array is modeled by a separate encoder. 
On top of the per-encoder attention mechanism, hierarchical attention network is employed to focus on the array stream that generates more informative higher-level representations. 
At the same time, each encoder is associated with a CTC network to guide the frame-wise alignment process, in order to potentially achieve the best results. 




Two parallel encoders with heterogeneous structures, RNN-based and CNN-RNN-based, are mutually complementary in characterizing the speech signal. 
Inspired by the advances in Hierarchical Attention Network (HAN) in document classification and multi-model video description, we adapted HAN into our MEMR model.  
The encoder that carries the most discriminate information for prediction could dynamically receive a stronger weight.  
Each individual encoder is associated with a CTC network to guide the frame-wise alignment process.
We evaluated the use of the MEMR model on WSJ and CHiME-4 and our MEMR model showed significant relative improvement of $18-32.1\%$ over related models with single encoders. 

==> outline.tex <==
% abstract done

% sec1. Introduction: done
% 1. explain the multi-array setting and difficulties, and stress the importance of the information fusion of this setting in terms of robustness, and how different this task is from multi-channel -- xiaofei
% 2. prior work in conventional ASR (multi-array and multi-channel work). Specially, how fusion is done.  (front-end fusion, back-end fusion, posterior fusion, PM) -- xiaofei
% 3. description of end-to-end approach and its advantage. Introduction of joint e2e model.  --ruizhili 
% 4. prior work in e2e (multi-array and multi-channel). specially, how fusion is done(frame-level fusion(multi-head), context vector level fusion(HAN)) --ruizhi
% 5. our introduce (hierarchical attention network) HAN in joint e2e model. (highlight: 1. multi-encoder for multi-array setup 2. HAN for robustness, 2. joint model with per-encoder ctc helps with ctc in general) -- xiaofei


% sec2. joint model   -- done
% 1. big picture 
% 2. pros and cons of ctc and attentin 
% 3. training :joint loss function 
% 4. decoding: joint decoding with rnnlm


% sec3. proposed model (han in joint model framework) --ruizhi 
% 1. big picture 
% 3.1-2. multi-encoder with HAN (we explore two kinds of encoder structure)
% 3.3. joint model with per-encoder CTC (explain training and decoding with RNNLM)


% sec4. experiment and discussion  -- xiaofei
% 1. data (AMI and DIRHA) done
% 2. experiment setup done
% 3. results 
% 3.1.single stream results with multi-stream 
% 3.2 multi-stream compared other approach 
% 3.3 stream attention robustness (stronger noise?)
